MASR: A Modular Accelerator for Sparse RNNs

Recurrent neural networks (RNNs) are becoming the de facto solution for speech recognition. RNNs exploit long-term temporal relationships in data by applying repeated, learned transformations. Unlike fully-connected (FC) layers with single vector matrix operations, RNN layers consist of hundreds of such operations chained over time. This poses challenges unique to RNNs that are not found in convolutional neural networks (CNNs) or FC models, namely large dynamic activation. In this paper we present MASR, a principled and modular architecture that accelerates bidirectional RNNs for on-chip ASR. MASR is designed to exploit sparsity in both dynamic activations and static weights. The architecture is enhanced by a series of dynamic activation optimizations that enable compact storage, ensure no energy is wasted computing null operations, and maintain high MAC utilization for highly parallel accelerator designs. In comparison to current state-of-the-art sparse neural network accelerators (e.g., EIE), MASR provides 2x area 3x energy, and 1.6x performance benefits. The modular nature of MASR enables designs that efficiently scale from resource-constrained low-power IoT applications to large-scale, highly parallel datacenter deployments.

==> PPA.tex <==
 \begin{figure*}[t]
    \centering
    \subfloat[Performance benefits for each optimization normalized to the platform running a distilled network.]{{\includegraphics[width=0.5\linewidth]{plots/perf_opts_top_down.pdf} }}%
    \subfloat[Area breakdown per accelerator over each stage of optimization.]{{\includegraphics[width=0.5\linewidth]{plots/area_breakdown.pdf} }}%
    \linebreak
    \subfloat[Energy breakdown per accelerator over each stage of optimization]{{\includegraphics[width=0.5\linewidth]{plots/energy_breakdown.pdf} }}%
    \subfloat[Power breakdown per accelerator over each stage of optimization]{{\includegraphics[width=0.5\linewidth]{plots/power_breakdown.pdf} }}%
    \caption{}%
    \label{fig:ppa}%
\end{figure*}

\section{Power, Performance, Area} \label{sec:ppa}
In this section we discuss the energy, power, area, and performance benefits of each optimization shown in Figure \ref{fig:ppa}.
Here we consider accelerator design ranging from 32 to 1024 parallel lanes.
Each design considered is a point on the energy-performance and area-performance Pareto-frontier shown in Figure \ref{fig:pareto}.

Figure \ref{fig:ppa}a illustrates the ratio of performance benefits each optimization offers for programmable CPU and GPUs as well as the considered accelerator designs.
As expected knowledge distillation improves the performance for all platforms by 1.4$\times$.
This constitutes a larger ratio of performance improvement measured on CPUs and GPUs as these platforms are unable to efficiently leverage dynamic activation sparsity and speculative output execution.
Similarly, we find that sparse weight execution constitutes a larger ratio of the speedup on less parallel accelerator designs such as the 32 lane topology as compared to the 1024 lane design.
This is a result of increased load imbalance seen in the larger designs.
% Should we go back and talk about the fact that after weight sparsity each lane does ~7 MACs per output neuron? Adding activation sprarsity brings this down to 2 - causing severe load imbalance.
For instance, on the largest design, Accelx1024, we find that with sparse weight execution each lane compute on average 7 MACs per output neuron.
These few operations are further reduced when considering sparse activations to 2 MACs on average.
The benefits of sparse activation execution and output speculation are thus diminished by high load imbalance across lanes.

Figure \ref{fig:ppa} b illustrates the area consumption of each accelerator design.
Following the area-performance Pareto-frontier shown in \ref{fig:pareto}, we see that larger accelerator designs consume more area as the area-efficiency on the weights and weights mask SRAMs decreases.
We also see that the area consumed by registers and logic increases for larger designs.
This increase is dominated (over 90\%) by the increase in registers needed to store the weights and activation bitmasks per lane - an overhead of sparse weight and activity execution and storage.
The secondary source (around 8\%) of register area are the queue between each lane and the backend accumulators. 
Noe that as knowledge distillation simply reduces the number of layers, is has no impact on on-chip area.

Figure \ref{fig:ppa} c and d illustrates the energy and power consumption of each accelerator design.
We find that, despite having smaller SRAMs for the largest Accelx1024 design, the design with the lowest energy consumption is actually Accelx256.
The reason for this is two-fold: (1) energy efficiency per read operation plateaus for more parallel accelerator designs, and (2) the power consumed by registers becomes more prominent for larger accelerator designs.
The first reason, as previous discussed in Section \ref{sec:pareto}, is a result of smaller memories for the Accelx512 and Accelx1024 designs not providing substantial reductions in dynamic power consumed by read operations.
The second, as shown in Figure \ref{fig:ppa}c, is a result from the increase in register power for more parallel design.
Once again we find that close to 99\% of the register power is consumed by the pipeline registers and maintaining bit-masks for the sparse execution and storage.

\subsection{Double Buffering Weights}
In order to minimize the required memory stored on-chip, weights for the forward and backward pass are double buffered. 
That is, while the \NAME accelerator executes the forward pass the weights for the backward pass are loaded in parallel from an off-accelerator memory.
Similarly, while executing the backward pass the weights for the next layer's forward pass can be loaded in parallel.
Here, we investigate the performance the performance and energy overheads of double buffering weights from an off-accelerator memory. 

As an example lets assume, LPDDR4 is used as an off-accelerator memory unit.
At 25.6GB/s of bandwidth and an average power of 200mW \cite{drampower}, we find that it takes 0.019ms and 3.8uJ to load the weights for a single direction.
In comparison, the most energy efficient accelerator design, \NAME x256, takes 0.14ms and consumes 38 uJ of energy to process 4 seconds of speech data for a single direction and layer.
That is, using LPDDR4 to double buffer the weights takes around 14\% of the time of running the RNN computation and 10\% of the energy.
Naturally processing shorter speech samples reduces the reuse in weights and will decrease the fraction of energy devoted to running the computation versus pre-fetching weights from an off-accelerator memory like LPDDR4.

% \begin{itemize}
% \item In terms of energy we find that the optimal design point is the Accelx256. This is because after that point energy efficiency plateaus for the SRAMs and the overhead of registers (check) causes the Accelx512 and Accelx1024 becomes more prominent.
% \item In terms of power we note that the optimizations have more of a benefit on larger accelerator topologies as for smaller accelerators the energy is dominated by SRAM memories. Though the optimizations reduce the SRAM area which you would expect to reduce the energy consumed, they end up just decreasing the number of maximally sized SRAM (set by the ARM memory compiler). This does reduce the leakage power, however since this is small compared to the dynamic read energy it has a small impact. 
% \item DRAM power becomes more prominent for larger accelerator topologies as the execution time is much smaller so the average power is amortized on slower designs.
% \item The power is largely determined by the weight SRAMs, weight mask SRAMs, and accesses to the compact activation register files. 
% \end{itemize} 

==> ds2.tex <==


%\begin{figure}[t]
%\center
%\includegraphics[width=\linewidth]{figures/flow.pdf}
%\centering
%\caption{Overview of the optimizations and benefits demonstrated.
%Each proposed technique (blue rounded rectangle) is labeled with the corresponding %contribution \fixme{in Table~\ref{tab:novelty}}. }
%\label{fig:flow}
%\vspace{-1em}
%\end{figure}


\section{Automatic Speech Recognition}

We begin with a background on automatic speech recognition (ASR).
Speech recognition aims to automatically transcribe an input $x$ into text $y$.
Throughout we will assume the input speech samples $x$ are represented as a discrete time series of continuous feature vectors $x^1, \ldots, x^T $.
The input features are derived from a spectrogram of power normalized audio clips (e.g., mel-frequency cepstral coefficients).
Current state-of-the-art models for ASR rely heavily on deep learning approaches for the acoustic modeling problem \cite{mohamed2012acoustic,hinton2012deep}.
Recently RNNs have become standard for end-to-end deep learning approach for modeling speech signals \cite{ds2,sak2014long}.
We first introduce recurrent neural networks and then describe how they are employed in speech recognition.
\fixme{Then we talk about optimizing baseline RNNs using model compression techniques including: Knowledge distillation, weight pruning, quantization.}
 % such as Deep Speech 2\cite{ds2}.

\subsection{Recurrent Neural Networks}
\fixme{Talk about GRU/LSTM vs. RNN; Unidirectional vs. bi-directional (Figure 3); Define recurrent neural network vs. RNN vs. GRU vs. LSTM (when we say RNN we mean vanilla RNN)}
Recurrent neural networks layers specialize in building long-term
context in time series data using a recurrent hidden state.
By maintaining and updating the hidden state across many
timesteps, recurrent layers can learn feature patterns in long-term
data. This property is useful in many language problems such as speech
recognition.

% successive input timesteps using a recurrent hidden
% state, $h^t$.
\begin{figure}[!t]
\includegraphics[width=\linewidth]{figures/bidir-rnn.pdf}
\centering
\caption{Architecture of bi-directional RNN layer where the input
  intermediates (red) and hidden intermediates (blue) after the
  respective matrix-vector products are highlighted. $x^t$ represents
  an input at timestep $t$. $h^t$ and $g^t$ represent the
  hidden-states for the forward and backward directions at timestep
  $t$. $W^x$, $W^h$, $V^x$, and $V^h$ are the forward and backward weight
  parameters; each of these is an 800x800 matrix.}
\label{fig:rnn}
\vspace{-1em}
\end{figure}

\input{tables/ds2_table.tex}

There are three popular classes of recurrent layers: vanilla RNNs,
gated-recurrent units (GRU) \cite{chung2014empirical}, and long-short
term memory (LSTM) networks \cite{hochreiter1997long}.  The layers differ in how they
update the hidden state based on seeing new input. RNNs use a standard
neural connection to combine a new input and the current hidden
state. GRUs and LSTMs are extensions of standard RNNs targeted at
learning longer term context. They achieve this through updates with
gated skip connections that control the flow of gradients.  For
example, GRUs have two gates that correspond to resetting and updating
the state, respectively, whereas LSTMs have three separate gates.
Though GRUs and LSTMs can typically achieve higher accuracy than
vanilla RNNs, the additional components require 3$\times$ and
  4$\times$ more parameters and operations than RNNs.
% We should define hidden units.

Each of these RNN types can be used in either a uni-directional or
bi-directional manner.  Uni-directional recurrent layers build the
hidden state based entirely on information from previous timesteps.
Bi-directional recurrent layers instead maintain two separate hidden
states, one based on inputs samples from the past and one based on
input samples from the future.  Though bi-directional layers can
achieve higher accuracy by leveraging information from the past and
future, they have twice the number of parameters and operations
as uni-directional layers.



\begin{figure}[!t]
\includegraphics[width=\linewidth]{plots/distill.pdf}
\centering
\caption{After distillation, a student 5 layer bidirectional RNN
  reaches the performance of a 7-layer bi-directional RNN or a 5-layer
  bi-directional GRU saving 1.4$\times$ and 3$\times$ the number of
  parameters respectively.}
\label{fig:distill}
\vspace{-1.25em}
\end{figure}

Figure~\ref{fig:rnn} illustrates the architecture of a bi-directional
vanilla RNN layer. Here $x^t$ is one \textit{input} to the
layer. First a batch norm regularization step is applied (discussed
more in the next section) \cite{ioffe2015batch}. Then the input is
transformed by matrices $W^x$ and $V^x$ to produce \textit{input
  intermediates} (shown in red). Simultaneously the neighboring hidden
states $h^{t-1}$ and $g^{t+1}$ are transformed by matrices $W^h$ and
$V^h$ to produce forward and backward \textit{hidden intermediates}
(shown in blue). The input and hidden intermediates are
accumulated and a sparsifying ReLU non-linear activation function is
applied to produce the new hidden states $h^t$ and $g^t$. These hidden
states are summed to create output $y^t$ and passed to the
next layer.

%  into both a left-to-right RNN to produce hidden state
% $h^t$ and a right-to-left RNN to produce $g^t$.

% Here there are effectively two RNNs one with hidden
% state $h^t$ and one with hidden state $g^t$. The first state is
% updated in a right-to-left manner and the second
% left-to-right.

% \begin{itemize}
% \item Talk about the figure and in particular we want to define
%   inputs, hidden-state, input intermediates, hidden intermediates.
% \item Intermediates are the outputs of each matrix-vector product but before the accumulation.
% \end{itemize}


\subsection{Target Model: Deep Speech 2}
\fixme{Brief overview of Deep SPeech; each layer is 800x800; CNN is not very costly and do not harp on NVDLA too much. beam search vs. greedy decoder; Start with a baseline trained in PyTorch and then next section optimizes the model}
To study deep models of speech recognition, we will focus on the the
popular Deep Speech~2 architecture~\cite{ds2}.  The Deep Speech~2
model is a multilayer neural network that maps from an input signal
directly to character predictions.

Table~\ref{tab:ds2} summarizes the Deep Speech~2 architecture.  The
model consists of a mix of convolutional, recurrent, and
fully-connected layers. First a pair of convolutional layers are
applied in the frequency-and-time domain (2D). Like convolution
filters found in DNNs for image classification and vision
applications, these layers learn local temporal relations translations
and also act to shorten the inputs through subsampling.  Next a series
of recurrent layers is applied.
These can either be GRU or vanilla RNN layers~\cite{ds2}.
Finally a fully connected layer is applied to make
output predictions in the form of scores for each possible
character. The final output of this model is a probability
distribution for the spoken character at each timestep.  The time
series probability distribution can then be fed into a decoder that
produces the final transcribed text by combining these
with a language model step.

In this work we focus on optimizing the RNN layers of this model.  In
both variants of the model, over 99\% of the parameters in the network
are found in the recurrent layers, as shown in Table~\ref{tab:ds2}.
We also note that the convolutions can be readily accelerated by
previous work on CNN accelerators. For instance, the open-source
NVDLA~\cite{nvdla} accelerator with 256 multipliers takes around 11 ms
to process an average sample from our data set. For our comparisons we
also consider a fixed length input signal of 7 seconds, the average
length in our dataset. For longer sequences, the forward states can be
used exactly and backward context can be computed by a small
overlapping window. Finally note there are two common approaches to
decoding from the predicted distribution: greedily or using beam
search.  For the purposes of this study, all the networks assume a
greedy decoder. While language model and beam search decoding further
improve performance, these steps can be performed after the output of
the system and their optimization is orthogonal to the main predictive
bottleneck.

% To further simplify our
% setup, we consider

% . Thus, in this paper we focus
% on building specialized hardware for the recurrent layers of
% Deep Speech~2.



%  Recent work has
% also shown that beam-search decoding provides marginal benefits in
% model accuracy~\cite{ds3}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/encoding.pdf}%
    \caption{ Encoding scheme based on binary masks }
    \label{fig:encoding}%
    \vspace{-1em}
\end{figure}


\NAME\ starts by training this baseline model for speech recognition.
To ensure the models achieve state-of-the-art accuracy, \NAME\ uses
models on top of the open-source Deep Speech~2 \cite{seannaren}
implementation in Pytorch~\cite{pytorch}. The models are trained with
the Connectionist Temporal Classification (CTC) loss
function~\cite{ctc} on the open-source LibriSpeech corpus \cite{libri}
containing over 1000 hours of speech data.  The RNN and GRU networks
start with baseline word-error rates (WER) of 21.3 and 21.2,
respectively.  Note that these results are comparable to the proposed
Deep Speech~2 networks using a greedy decoder and without a language
model~\cite{ds2}.

% To train the Deep Speech 2 model we use the open-source LibriSpeech
% corpus \cite{} that consists of over 1000 hours of spoken data along
% with the CTC loss function \cite{ctc}. While this score is below the
% performance of industrial grade datasets, it is competitive with the
% numbers reported in DeepSpeech 2 on similar sized data.

%  on NVIDIA GTX 1080 Ti
% platforms.

% In particular, we will study bi-directional RNNs.


% \begin{itemize}
% % \item There is acoustic model and language model. We focus on acoustic
% %   model and greedy decode.
% \item Cite TPU to show that memory is the main bottle neck for these
%   RNN/LSTM based networks.
% \end{itemize}


==> dvfs.tex <==
% Introduce the fact that the accelerator runs really fast compared to what we need for speech recognition. Thus here investigate if we can tradeoff performance for energy, or power - important for real-time embedded devices.


\section{Scalability of Disciplina}
\label{sec:scale}
As voice-based human machine interfacing continues to be used by more services,
ASR is expected to be deployed across a spectrum of platforms ranging from
high-performance cloud-based services to deeply-embedded, resource-limited edge and IoT devices.
This section demonstrates how \NAME\ offers a scalable solution across a wide range of platforms.

In situations that require \textbf{high performance and throughout} (e.g., cloud-based ASR services), the LANESx1024 scale-up design can process 7$s$ of speech in 0.72$ms$ while consuming 472$\mu J$
and dissipating 652$mW$. This provides more than sufficient latency for cloud-based speech APIs.

On the other hand, for \textbf{resource constrained edge devices}, energy consumption and thermal design
power (TDP) are first-order constraints. These applications are typically user-centric and latency of a single ASR request is paramount. LANEx256, the energy optimal design from Section~\ref{sec:dse},
processes 7 seconds of speech in 1.39$ms$ while dissipating 270$mW$ of power and consuming 375$uJ$ of energy.
Taking real-time constraints into account, we find additional opportunity to optimize the accelerator's power and energy.


As bi-directional RNN operates on an entire sample of speech in the forward and reverse directions, a standard frame-by-frame definition of real-time execution based on audio sampling rates is not applicable. Instead, we define real-time requirements for ASR by acceptable quality-of-service latencies.
%International communication
%standards state humans can tolerate response latencies on the order of 10s of milliseconds of audio to visual delay without noticeably impacting QoS. In particular,
For example, the International Telecommunication Union defines acceptable mouth-to-ear latency for highly interactive applications, such as speech, to be 100$ms$ (ITU 2003).
%
%This provides additional opportunities for real-time ASR applications
%(e.g., personal assistants, mobile devices, wearables)
%the performance requirements are inordinately low.
%while meeting the requirements for real-time speech recognition, to improve energy
%efficiency and power consumption.
%
The LANEx256 accelerator processes the average speech duration of the LibriSpeech dataset 40$\times$ faster than the 100$ms$ requirement for real-time speech recognition.
%This slack can be exploited with voltage and frequency scaling to maximize energy efficiency.
Figure \ref{fig:dvfs} illustrates the overall energy consumption of all Pareto optimal designs when scaling voltage of the proposed accelerator from the nominal $0.8$V down to $0.54$V, the minimum supply voltage for conventional SRAM memories.
After scaling voltage, we find that the critical path is in the logic and not the SRAM memories. At 0.54$V$, clock frequency decreases from 1GHZ to 285 MHz.
%For each new voltage and frequency operating condition,
%we re-characterized the SRAM memories used by our simulator to appropriately model
%accelerator performance, power, and energy.
Figure \ref{fig:dvfs}a shows that at the lowest operating voltage,
the energy consumed by each accelerator design reduces by a factor of 1.76$\times$.

Even after scaling voltage to the minimum 0.54$V$ and frequency to 285$MHz$,
\NAME\ still comfortably meets real-time ASR requirements.
%To further reduce power, we can further reduce frequency while keeping voltage constant.
For energy-optimal LANESx256, we can further reduce frequency down to 15$MHz$, meet real-time requirements, and only consume 3.6$mW$.
%However, reducing frequency alone only saves dynamic read power, and SRAM leakage power becomes prominent in the accelerator's overall power footprint. Compared to running at 285$MHz$, the 15$MHz$ and 3.6$mW$ design consumes 1.1$\times$ more energy. As was the case in Section~\ref{sec:dse}, the optimal point depends on the application; the voltage frequency case study presented here provides optimal energy and power design points to suit different use cases.


%by 1.76$\times$ (214 $uJ$) and 74$\times$ (3.6$mW$) respectively.
%Operating under this low of a power envelope barely registers on many embedded devices with TDP on the order of watts.
%This makes deploying \NAME~ in embedded devices non-intrusive;
%the orchestration of running \NAME~ in parallel with other IP blocks is unlikely
%to exacerbate or introduce any dark or dim silicon effects\fixme{~\cite{}}.


%\textbf{Defining Real-Time Constraints}
%We begin by defining the real-time requirements for speech-recognition.
%As bi-directional RNN operates on an entire sample of speech in the forward and reverse directions,
%a standard frame-by-frame definition of real-time execution based on audio sampling rates is not applicable.
%Instead, we define real-time requirements for ASR by acceptable quality-of-service latencies.
%In particular, the International Telecommunication Union defines acceptable mouth-to-ear for highly interactive applications, such as %speech, as 100$ms$ (ITU 2003).
%Thus, for the purposes of this study, we set the real-time requirements for ASR to be 100$ms$.
%Similarly, the European Broadcasting Union limits the lag delay of sound after picture to be a more aggressive 60$ms$.
%For the purposes of this study, we set the real-time requirements of speech recognition to be 60$ms$.
%\fixme{Should we cite Glenn's paper and say that this is a more aggressive form of what they assumed which was 200 ms?}


%\subsection{Scaling Voltage and Frequency}
%The LANEx256 accelerator processes the average speech duration of the LibriSpeech dataset (7 seconds) in 1.39$ms$.
%This is 40$\times$ faster than the 100$ms$ requirement for real-time speech recognition.
%Here we apply voltage and frequency scaling to claim
%additional energy and power benefits while meeting the real-time requirements.
%To improve computational efficiency, we use this slack to reduce power and energy
%with voltage and frequency scaling.

%Figure \ref{fig:dvfs}a illustrates the overall energy consumption of all Pareto optimal designs
%when scaling the voltage of the proposed accelerator.
%Here, voltage is scaled from a nominal 0.8V down to $0.54$V,
%the lowest voltage supported by the available SRAM memories.
%When scaling voltage,
%we find the critical path is in the logic and not the SRAM memories.
%At 0.54$V$ the clock frequency decreases from 1GHZ to 285 MHz.
%For each new voltage and frequency operating condition,
%we re-characterized the SRAM memories used by our simulator to appropriately model
%accelerator performance, power, and energy.
%Figure \ref{fig:dvfs}a shows that at the lowest operating voltage,
%the energy consumed by each accelerator design is further reduced by a factor 1.76$\times$.
%\fixme{Replot as bars. make note about how max parallel still isnt most efficient. there's another dark Si argument to be made here.}
%At nominal 0.8$V$ the critical path in the accelerator design was set by the logic at 1GHz.
%The SRAM memories can operate at a slightly higher frequency of 1.25 GHz.
%Thus, to determine the frequency of the accelerator running at different voltages, we measure the impact of voltage scaling on the delay of the logic.
%Thus, in order to scale the voltage and frequency, we measure the impact of voltage scaling on the delay of the logic.
%The power for the SRAM memories and logic is re-characterized for the new voltage and frequency.
%The lowest voltage supported by the available TSMC 16nm FinFet SRAM memories is 0.54$V$.
%The clock frequency at 0.54$V$ is scaled from the nominal 1$ns$ to 3.5$ns$.
%At this point, we find that the overall energy consumption of the accelerator is reduced by a factor of \fixme{1.7$\times$}.

%Even after scaling the voltage to 0.5$V$ and the frequency to $285$MHz,
%\NAME\ still comfortably meets the real-time ASR requirements.
%To further reduce the power consumed, we scale frequency while keeping the voltage constant.
%We find that for the energy optimal design point, LANESx256, we are able to scale the frequency down to 15 MHz and still meet the performance standard.
%Operating at this 0.54$V$ and 37MHz results in the accelerator to have a power budget of a mere 3.6$mW$.
%However, by reducing frequency alone, only dynamic read power is saved and SRAM leakage power becomes prominent in accelerator's overall power footprint.
%Compared to running at 285MHz, the 15MHz, 3.6$mW$ design consumes 1.1$\times$ more energy energy.
%As was the case in Section~\ref{sec:dse}, the optimal point depends on the application;
%the voltage frequency case study presented here provides optimal energy and power design points to suit different use cases.
%Despite this small penalty, integrating \NAME\ into a deeply-embedded device would enable real-time on-chip speech recognition at a small energy footprint and negligible increase in TDP.


==> overview.tex <==



\section{Overview}
In this section we give a brief overview of each stage of the holistic co-design flow illustrated in Figure \ref{fig:flow}

\subsection{Static Model Optimizations} 
\paragraph*{\textbf{Knowledge distillation}}
\NAME first uses knowledge distillation to compress bi-directional RNN and GRU based networks in terms of their size and number of layers.
This stage uses a pre-trained baseline, \textit{teacher}, network to train a smaller, \textit{student}, network while maintaining comparable accuracy to the baseline.
Of the possible networks, \NAME picks the network with the fewest number of parameters, a 5-layer bi-directional RNN, that achieve reasonable accuracy. 
The benefits of compression are applicable to all platforms considered including CPUs, GPUs, and specialized hardware. 

\paragraph*{\textbf{Weight Pruning}} The distilled bi-directional RNN is then pruned to further reduce the storage requirements.
\NAME uses threshold based magnitude pruning to eliminate parameters while maintaining comparable accuracy to the distilled model. 
The proposed accelerator leverages binary sparse encoding to eliminate wasted work with low storage overhead, and to enable speculative output neuron execution. 

\subsection{Dynamic Activation Optimizations}

\paragraph*{\textbf{ReLu Thresholding Hidden-State}}
Leveraging the ReLu non-linearity in the distilled and pruned bi-directional RNN, \NAME enables sparse storage and execution of the hidden-state.
In order to reduce the intermediate storage, \NAME computes each timestep sequentially as opposed to evaluating the matrix-vector products for all inputs in parallel.

\paragraph*{\textbf{Refactoring Batch Normalization for Sparse Inputs}}

Based on characteristics gathered during training, batch normalization scales and translates the inputs to each layer to have zero mean and unit variance.
Though batch normalization provides better training accuracy, it also transforms sparse inputs to dense ones.
To recover sparsity, \NAME refactors the batch norm operation into the subsequent RNN layer's weights and biases.
The refactoring can be done off-line without any run-time execution overhead.
This enables sparse input execution and compact activity (hidden-state and input) storage.

\paragraph*{\textbf{Speculative Execution for Output Neurons}}
Given that the inputs to each layer undergo batch normalization, the distribution of the inputs and hidden-state are quite distinct. 
In particular the hidden-state intermediates tend to be more negative than the input intermediates.
We leverage this distinction, and the fact that ReLu thresholds away negative values, to predicate the computation for output neurons corresponding to the input matrix-vector operations, based on the hidden-state intermediates. 
We find that up to 30\% of the input matrix vector product computations can be speculatively skipped using a low-cost dynamic threhsolding mechanism. 

\subsection{DVFS for Real Time Execution}
We find that the proposed hardware accelerator comfortably meets requirements for real-time speech recognition.
To save energy we apply DVFS.
To reduce power at iso-energy, we scale the frequency until the design meets requirements for real-time speech recognition.

==> related_work_orig.tex <==

\section{Related Work}
% \fixme{Short paragraph on ASR models - HMM's and RNNs. \cite{unfold}, \cite{price} }
% The last two do DNN+Viterbi and WSFT models. We focus on RNN based ASR which is the state of the art currently. 

%\input{tables/comparison}
Deep neural networks entail a general class of machine learning models that have been deployed across a wide set of applications and platforms~\cite{hpca2018amlfb,fathom,isca2017tpu}.  Given their ability to achieve state-of-the-art accuracy in a broad range of applications, DNNs have gained a lot of attention from the architecture community \cite{diannao,dadiannao,eie,eyeriss,minerva,cambricon,scnn,cnvlutin,epur,circnn,isaac,DBLP:journals/corr/RhuOCPK17}.
Several of these works leverage network sparsity to improve the performance, area, and energy efficiency of DNN inferences.
The authors of~\cite{minerva} demonstrate that up to 95\% of all computations can be skipped by pruning small activations without loss in accuracy. Moreover, advanced task skipping techniques such as PredictiveNet~\cite{predictivenet} and SnaPEA~\cite{SnaPEA} have been shown to deliver further speedup and energy improvements during CNN inference by cutting or abandoning the computation if the output has been speculated to be negatively valued as ReLU will zero out. \NAME\/'s predicated neuron execution is customized to RNNs but similar in spirit to these techniques in the sense that neuron execution is skipped if the corresponding hidden intermediates are sufficiently negative.

Previous works accelerating sparse neural networks have focused on optimizing the computation in fully-connected~\cite{eie} or convolutional layers~\cite{eyeriss,scnn,cambricon,cnvlutin}. To reduce the on-chip storage and the energy cost of data movement, these accelerators shrink the parameter space by way of run-length sparse encoding. 
%For example, the reconfigurable CNN accelerator Eyeriss~\cite{eyeriss} clock-gates the PEs on null activations but still performs multiplication on zero-valued weights. 
%\fixme{The SCNN accelerator~\cite{scnn} uses a run-length encoding scheme to store the sparse weights and activations in a compressed representation and saves the multiplier from operating on null operands.}
%The Cambricon-X~\cite{cambricon} accelerator exploits the sparsity in weight only, leaving activations unpruned, and employs a step indexing scheme also based on run-length encoding. 
In contrast, \NAME\ focuses on accelerating the computation in RNN layers where the ratio of activations to weights is typically higher than in FC or CNN layers. Moreover, unlike run-length encoding, \NAME\ employs a binary mask encoding scheme which is agnostic to the distribution of sparse values, and not only enables skipping computations on both null weights and activations, but also facilitates the compact storage of non-zero elements in memory. Therefore, \NAME's encoding scheme effectively prohibits wasted work.  

%\fixme{Explain why we compare with EIE/ESE annd E-PUR and not all the others}
%In this paper, we compare~\cite{eie} to the proposed \NAME\ design.

%In addition to eliminating redundant parameters, other work has investigated techniques to leverage the inherent fault tolerance of DNNs.
%For instance, \cite{temam,dengretime} illustrate that DNNs can be retrained to mitigate the impact of performance faults.
%In~\cite{minerva}, the authors illustrate that Razor SRAM fault mitigation techniques can enable power savings by reducing the voltage supply to SRAMs.
%\NAME\ proposes speculative execution, a low-cost solution that enables predicating up to 30\% of the input vector-matrix multiplications in RNNs.
In addition to building accelerators for DNNs and CNNs, other work has investigated RNNs and search algorithms to target domains such as ASR and machine translation. For use in an end-to-end ASR system, the authors of~\cite{unfold} designed a memory-efficient accelerator primarily targeted to accelerate the Viterbi search after the processing of RNN layers. ~\cite{congrnn,eugeniornn,drnn} leverage the temporal locality of RNNs to accelerate them on FPGAs. Memoizing the input vector-matrix multiplications in RNNs for language modeling is proposed in~\cite{fpl2016intel}. However, given the large variance in input speech samples, this is infeasible for ASR. ESE~\cite{fpga2017esehan} proposes a sparse weight RNN accelerator based on the pruning method discussed in~\cite{iclr2016deepcompression}. E-PUR~\cite{epur} provides a technique for maximizing weight locality in RNNs, but it performs dense computations on densely stored representations. Section~\ref{sec:discuss} compared \NAME\ to the end-to-end sparse accelerators in~\cite{eie} and~\cite{fpga2017esehan}.






==> tables/comparison.tex <==
\begin{table}[t!]
  \begin{center}
    \caption{
Comparison of \NAME\ with related work.
%All networks are trained for a total of 20 epochs (like the Baidu paper \cite{ds2}. For knowledge distillation we only use the teacher networks logits for the first 10 epochs and then switch over to the one-hot encoded training set.
             }
    \label{tab:comparison}
    \begin{tabular}{c|c|c|c}
     \toprule	
      & SRAM & Area & Energy \\
      & (MB) & (mm$^2$) & ($\mu$J) \\ \hline
    E-PUR \cite{epur}  & 7.3 & 10.1   & 4425 \\   \hline
    ESE \cite{fpga2017esehan} & 3.6 &  5.0   & 1725 \\   \hline
    {EIE \cite{eie}}  & 3.6  & 5.0  & 1162 \\  \hline
    \NAME (LANESx256) & 1.8  & 2.5   & 375\\  \hline
%     \NAME  & \multirow{2}{*}{1.8} &   \multirow{2}{*}{2.5} & 228 \\
%     (Real-Time)  & &   & (3.6mW)\\  \hline
   \end{tabular}
  \end{center}
  \vspace{-1.5em}
\end{table}


==> tables/novelty_table.tex <==
\begin{table*}[h!]
  \small
  \begin{center}
    \caption{
             \textbf{Proposed optimizations compared to related work.}
            }
    \vspace{-1em}
    \label{tab:novelty}
    \begin{tabular}{c@{\TABSEPsmall}|c@{\TABSEPsmall}c@{\TABSEPsmall}c@{\TABSEPsmall}c@{\TABSEPlarge}?c@{\TABSEPsmall}|l@{\TABSEPlarge}}
     \toprule
     Technique &\cite{fpga2017esehan} & \cite{eie} & \cite{epur} & \cite{cambricon} & This Work & \multicolumn{1}{c}{Contribution}  \\ \cmidrule{1-7}
     Knowledge Distillation &  &  &  &  & \ding{52} & C1: Reduce number of layers with no loss in accuracy. \\ \cmidrule{1-7}
     Weight Pruning & \ding{52}& \ding{52}& & \ding{52} & \ding{52} & C2: First to prune a distilled bi-directional RNN.  \\ \cmidrule{1-7}
     % Sparse Activity Execution
     Sparse Activity &  & \multirow{2}{*}{\ding{52}} & & & \multirow{2}{*}{\ding{52}} & C3: First to leverage ReLu for sparse hidden state.  \\
     Execution & & & & &  & C4: First to refactor batch normalization for sparse inputs at zero cost.\\ \cmidrule{1-7}


     % Sparse Activity Storage
     Sparse Activity Storage  &  &    &  &  & \ding{52} & C5: Efficient relative indexing for sparse activity address. \\ \cmidrule{1-7}

     % Output Speculation
     Output Speculation &   &  & & &  \ding{52}  & C6: First to speculatively skip output neurons. \\ \cmidrule{1-7}
     RNN  & \ding{52} & & \ding{52} &  & \ding{52} & C7: First to support Bi-RNN; timesteps with batch normalization.\\ \toprule
   \end{tabular}
  \end{center}
    \vspace{-1em}
\end{table*}

     % Sparse Weight Storage
     %& \multirow{2}{*}{Sparse Weight Storage}  & \multirow{2}{*}{\ding{52}} & \multirow{2}{*}{\ding{52}}  &  & \multirow{2}{*}{\ding{52}} & \multirow{2}{*}{\ding{52}} & C6: Enable efficient output speculation \\
    % &  &  & & &  &  &   C7: Efficient relative indexing for sparse weight address\\ \cmidrule{2-8}
%       & & & & & & C10: First to apply DVFS for real-time speech recognition \\ \toprule
     %\multirow{2}{*}{Weight Pruning} & \multirow{2}{*}{\ding{52}}& \multirow{2}{*}{\ding{52}}& & \multirow{2}{*}{\ding{52}} & \multirow{2}{*}{\ding{52}} & C2: First to prune a distilled bi-directional RNN.  \\

